The category of MSO transductions

MSO transductions are binary relations between structures which are defined using monadic second-order logic. MSO transductions form a category, since they are closed under composition. We show that many notions from language theory, such as recognizability or tree decompositions, can be defined in an abstract way that only refers to MSO transductions and their compositions.

==> ap-cartesian.tex <==
\section{Cartesian products}

\begin{myexample}[Cartesian products] \label{ex:pairing} How do we model a pair of structures as a structure? There are several ways to do it, and one of them is described later in this example. Before describing the exact construction, we recall the categorical notion of pairing: a \emph{Cartesian product} of two classes of structures $\Cc_1$ and $\Cc_2$ is defined to be a class of structures $\Cc_1 \times \Cc_2$, together with \mso transductions
    \[
    \begin{tikzcd}
    \Cc_1 &
    \Cc_1 \times \Cc_2 
    \ar[l,"\pi_1"]
    \ar[r,"\pi_2"'] &
    \Cc_2,
    \end{tikzcd}
    \]
    which are called \emph{projections},
    such that 
    \[ \forall f_1\ \forall f_2\ \exists! f
   \qquad  \begin{tikzcd}
    & \Dd 
    \ar[dl,"f_1"']
    \ar[dr,"f_2"]
    \ar[dd,"f"]
    \\
    \Cc_1 && \Cc_2 \\ 
    &\Cc_1 \times \Cc_2 
    \ar[ul,"\pi_1"]
    \ar[ur,"\pi_2"']
    \end{tikzcd}
    \]
    Although there might be several ways of defining Cartesian products, all solutions are isomorphic, as classes of structures. Below is a specific construction of Cartesian products, but due to their uniqueness, we do not need to look it into the details too much, as long as we know that they exist. For two structures $A_1$ and $A_2$, define the \emph{pair structure} $(A_1,A_2)$ as follows: take the disjoint union of $A_1$ and $A_2$, and add a unary relation which selects elements from the universe of $A$. The vocabulary of the pair structure is the disjoint union of the vocabularies of the two structures $A_1$ and $A_2$, plus a new unary relation. One can easily show that the class of such pairs, together with the naturally defined projections, is indeed a Cartesian product. 
   
    Similarly, our category also has co-products. 
   
    An interesting example is lists. For a class of structures $\Cc$, one can define a new class of structures $\Cc^*$, which satisfies 
    \begin{align*}
    \Cc^* \quad \text{is isomorphic to} \quad 1 + \Cc \times \Cc^*.
    \end{align*}
    We do not know if the above equation has a unique solution up to isomorphism, and if not, then how can the equation be strengthened so that it does have a unique solution.
    \end{myexample}

==> ap-connected-components.tex <==
\subsection{Connected components}
We now show that original tree decompositions are consistent with taking connected components. We begin by recalling the notion of connectivity for matroids. Define a \emph{circuit} in a matroid to be a set that is dependent, and is minimal inclusion-wise for this property. In this paper, circuits in matroids will play the same role as paths in a graph: they will be used to connect elements. This intuition is supported by the following fact~\cite[Proposition 4.1.2]{oxley2011matroid}: for every matroid, the relation ``there is an circuit that connects $x$ and $y$'' is transitive, i.e.~an element can be reached using either a single circuit, or cannot be reached at all. Equivalence classes of this equivalence relation are called \emph{connected components}. Connected components are also related to the following separation notion: define a \emph{separation} in a matroid to be a partition of the elements into two subsets $X$ and $Y$ such that a set $Z$ is independent if and only if the intersections $Z \cap X$ and $Z \cap Y$ are independent. The following lemma explains the connection between circuits and separations. 

\begin{lemma}\cite[Proposition 4.2.1]{oxley2011matroid}\label{lem:connectivity} Two elements of a matroid are in the same connected component if and only if for every separation they are in the same part.
\end{lemma}

 We extend connected components from matroids to multi-matroids as follows: the partition of a multi-matroid into \emph{multi-connected components} is the least equivalence relation that contains, for every independence relation in the multi-matroid, the corresponding partition into connected components. In other words, elements $x$ and $y$ are in the same multi-connected component if one can go from $x$ to $y$ in a finite number of steps, where in each step we can move within a circuit of the multi-matroid. (Here, a circuit of the multi-matroid is a circuit for one of the independence relations in the multi-matroid.) Unlike for matroids, in a multi-matroid one might need several steps, since the circuits of the different independence relations can be unrelated, and we cannot apply the fact that the ``same circuit'' relation for every matroid is transitive. 


\begin{lemma}\label{lem:connected-components}
 Let $\Cc$ be a class of multi-matroids of degree at most $k$. Then $\Cc$ has original tree decompositions if and only if the same is true for 
 \begin{align*}
 \setbuild{A}{$A$ is obtained by restricting a multi-matroid in $\Cc$ to a multi-connected component}.
 \end{align*}
\end{lemma}
\begin{proof}
 Let us write $\connected(\Cc)$ for the class in the statement of the lemma, i.e.~the structures that arise by taking some multi-matroid from $\Cc$ and restricting it to a single multi-connected component. 

 
 \begin{itemize}
 \item[$\Leftarrow$] We first show that if $\connected(\Cc)$ has original tree decompositions, then so does $\Cc$. In the proof, we work with multisets of structures, described as follows. If $A_1,\ldots,A_n$ are structures over a common vocabulary, then the corresponding \emph{multiset structure} is defined as follows: take the disjoint union of $A_1,\ldots,A_n$ and adding an equivalence relation $x \sim y$ which holds whenever $x$ and $y$ come from the same structure. If $\Dd$ is a class of structures, then we write $\multiset \Dd$ for the class of structures which arise by taking finite multisets of structures from $\Dd$. 
 
 Consider the following sequence of \mso transductions:
 \[
 \begin{tikzcd}
 \Cc 
 \ar[d,"\text{split into multi-connected components}"]
 \\ 
 \multiset(\connected(\Cc)) 
 \ar[d,"\text{compute tree decompositions for each multiset element}"]
 \\
 \multiset(\text{trees}) 
 \ar[d,"\text{join trees with a common root}"]
 \\
 \text{trees}
 \end{tikzcd}
 \]
 The transduction in the middle uses the assumption that $\connected(\Cc)$ has original tree decompositions. Each of the transductions is easily seen to be an original encoding, thus proving that $\Cc$ has original tree decompositions. 
 \item[$\Rightarrow$] We now show that if $\Cc$ has original tree decompositions, then so does $\connected(\Cc)$. This is an immediate corollary of Lemma~\ref{lem:residuals} and the observation that if a multi-matroid has degree $k$, then all of its multi-connected components are residuals that have degree at most $k$. 
 \end{itemize}
\end{proof}



==> ap-hom-ord-part.tex <==
\subsection{Homogeneous ordered partitions}
In Section~\ref{sec:using-an-ordered-partition} we showed that if we are given a multi-matroid $A$ together with an ordered partition of degree $k$, we could split the multi-matroid into the corresponding residual list $[A_1,\ldots,A_n]$, and combine the definable tree decompositions for the list items into a definable tree decomposition for $A$ itself. This raises the question: where do get the ordered partition from? This question is addressed below. We will describe a special kind of ordered partition, which we call homogeneous, and we will show that such ordered partitions can be defined in \mso, assuming that they exist. (Later in the proof, we will show that they exist.)


\begin{definition}[Homogeneous ordered partition]
    Let 
\begin{align*}
X_1 < \cdots < X_n
\end{align*}
be an ordered partition of the elements in a matroid $A$.
Define the \emph{index} of an element to be the number in $\set{1,\ldots,n}$ of the equivalence class containing the element. 
We say that the ordered partition  is \emph{homogeneous} if
\begin{enumerate}
    \item \label{it:interval-circuits} for every circuit, the indices used by the circuit form an interval in $\set{1,\ldots,n}$;
    \item \label{it:short-circuits} if two elements have indexes that differ by at most $\delta \in \set{0,1}$, then they can be connected by some circuit that visits at $\delta+3$ indices (i.e.~the two elements belong to some circuit that intersects at least $\delta+3$ equivalence classes).
\end{enumerate}
\end{definition}

A corollary of the second item is that the matroid has one connected component, since every two elements with consecutive indices can be connected by some circuit. 
The following lemma shows that homogeneous ordered partitions of constant degree can be produced by an \mso transduction. 
\begin{lemma}\label{lem:define-homogeneous-order}
    There is an original \mso transduction which inputs a matroid $A$, and outputs all possible pairs $(A,\le)$ such that $\le$ is a homogeneous ordered partition. 
\end{lemma}
\begin{proof}
    A simple modulo counting argument. Let $A$ be a matroid, and let $\le$ be a homogeneous ordered partition. Define the   \emph{colour} of an element to be its index (with respect to the ordered partition) modulo five. We will show that $\le$  can be described by only using its colours, as expressed in the following claim. In the claim, when we say that the indices of $x$ and $y$ differ by $\delta$, we refer to the difference in an asymmetric way: if $x$ and $y$ differ by $\delta$, then $y$ and $x$ differ by $-\delta$.
    

    


    \begin{claim}
        Let $A$ be a multi-matroid of degree at most $k$, and let $\le$ be a homogeneous ordered partition of degree at most $k$. Let  $\delta \in \set{0,1}$.  For every elements $x,y$ in the matroid,  the  following conditions are equivalent
        \begin{enumerate}[(a)]
            \item \label{it:index-delta} The indices of $x$ and $y$ differ by $\delta$. 
            \item \label{it:color-delta} The indices of $x$ and $y$ differ by $\delta$ modulo 5,  and there is some circuit that contains $x$ and $y$,  but avoids at least one colour.
        \end{enumerate}
    \end{claim}
    \begin{proof}
        \ 
        \begin{description}
            \item[\ref{it:index-delta}
             $\Rightarrow$ \ref{it:color-delta}] Assume~\ref{it:index-delta}. Clearly if the indices of $x$ and $y$ differ by $\delta$, then by item~\ref{it:short-circuits} in the definition of being homogeneous, one can connect $x$ and $y$  by a circuit that uses at most $\delta + 3 \le 4$ indices, and therefore avoids one of the five colours. 
            \item[\ref{it:index-delta}
             $\Leftarrow$ \ref{it:color-delta}] Assume~\ref{it:color-delta}. Since the colours of $x$ and $y$ differ by $\delta$, then their indices must differ by either $\delta$, or by at least four, as explained in Figure~\ref{fig:explain-mod-five}.
            The case that the indices differ by at least four is ruled out, since then any cycle connecting $x$ and $y$ would need to visit at least five consecutive indices -- and therefore all colours --  by condition~\ref{it:interval-circuits} in the definition of homogeneity. 
            \end{description}
    \end{proof}

\begin{figure*}
    \mypic{9}
    \caption{\label{fig:explain-mod-five} Red circles indicate the possible locations of $y$ so that the colours differ by $\delta=1$.}
\end{figure*}
      The second condition in the claim can be formalized by an \mso formula, which refers only to the independence relations in the matroid, and the five possible colours. Thanks to the claim, the relation ``the indices of $y$ and $x$ differ by either $0$ or $1$''
    can also be formalized by such a formula.
     The transitive closure of this relation describes the ordered partition, and since transitive closure can be defined in \mso, it follows that one can define any homogeneous ordered partition by an \mso formula that refers only to the independence relations in the matroid and the colours. The colours can be nondeterministically guessed by an \mso transduction, thus completing the proof of the lemma.
\end{proof}

\begin{corollary}\label{cor:equivalence-with-implicit-residual-lists}
    Let $\Cc$ be a class of multi-matroids of degree at most $k$. If $\Cc$ has  definable tree decompositions, then the same is true  for
    \begin{align*}
    \setbuild{ A}{ 
        $A$ is a multi-matroid of degree at most $k$,  such that\\ for some homogeneous  
        ordered partition $\le$ of degree  \\ at most $k$, the sequence of residuals is in $\Cc^*$
    }.
    \end{align*}
\end{corollary}
\begin{proof}
    By Lemma~\ref{lem:define-homogeneous-order}, the homogeneous ordered partition can be defined by an \mso transduction, if it exists. Therefore, we can apply Corollary~\ref{cor:equivalence-with-residual-lists}.
\end{proof}



==> ap-products.tex <==
\section{Products and co-products}
\label{sec:products-co-products}

==> defining-linear-orders.tex <==

\subsection{Multi-matroids}
In the proof, we will work with a slight generalization of matroids, which uses not one, but several independence relations on the same ground set.  

\begin{definition}[Multi-matroid]\label{def:multi-matroid}
    A \emph{multi-matroid} is a nonempty set of matroids, all of which have the same set of elements.
\end{definition}

We write $\mathbb A$ for multi-matroids, and $A \in \mathbb A$ for the matroids in them. A mult-matroid is called representable if all the matroids in it are representable (over our fixed field). Some of the results in this section will apply to general multi-matroids, and some only to those that are representable.

The \emph{degree} of a multi-matroid is defined to be the number of matroids in it. We assume that the degree is at least one. When the degree is exactly one, then a multi-matroid is the same thing as a matroid.  A multi-matroid of degree at most $k$ can be represented as a structure over the vocabulary
\begin{equation*}
\hspace{2cm}\myunderbrace{I_1(X),\ldots,I_k(X)}{names for the independence relations}.
\end{equation*}
We allow repetitions, i.e.~we do not require that the relations in this vocabulary are interpreted as distinct independence relations, and therefore multi-matroids of degree smaller than $k$ can also be represented.   When we talk about multi-matroids of degree at most $k$ as a class of structures in the context of \mso transductions, this is the representation that we use.   This representation is not unique, since we can choose the order and repetitions in which the independence relations are listed; more precisely if a multi-matroid has degree $\ell \le k$, then the number of representations over this vocabulary is the number of surjective functions $k \to \ell$. 


\subparagraph*{Using an ordered partition}
Define an \emph{ordered partition} in a set 
to be a binary relation $x \le y$ that is reflexive, transitive and total, which means that every two elements are comparable. An ordered partition  is the same thing as a partition of the set into equivalence classes $X_1,\ldots,X_n$, together with a linear order on its equivalence classes 
\begin{align*}
X_1 < \cdots < X_n.
\end{align*}
 We use the following terminology for ordered partitions: 
\begin{align*}
\myunderbrace{X_i}{equivalence class} 
\qquad 
\myunderbrace{X_1 \cup \cdots \cup X_i}{downset}
\quad 
\myunderbrace{X_i \cup \cdots \cup X_j}{interval, where $i \le j$}.
\end{align*}

We will be working with ordered partitions in a multi-matroid where every interval gives a residual of small degree. 

\begin{definition} The \emph{degree} of an ordered partition in a multi-matroid $A$  is defined to be the maximal degree of residuals obtained by restricting $A$ to some interval.
\end{definition}


The following lemma shows that a multi-matroid with an ordered partition of low degree can be recovered in \mso from the list of residuals of its equivalence classes. Before stating the lemma, we explain two items of notation used in it. 

We can also code lists of structures as structures. More formally, if $A_1,\ldots,A_n$ are structures over a common vocabulary, we define 
\begin{align*}
[A_1,\ldots,A_n]
\end{align*}
to be structure that is obtained by taking the disjoint union of the structures $A_1,\ldots,A_n$, and adding a binary relation $x \le y$ that describes the list order. We write $\Cc^+$ for the class of structures that arise this way, when all list elements are taken from some class $\Cc$. 

 In the lemma, by the \emph{inverse} of an original transduction we mean the original transduction obtained by swapping the input/output structures in each origin triple from the transduction. The inverse only makes sense for original transductions where the origin map is always a bijection.


\begin{lemma}\label{lem:reconstruct-multi-matroid-from-list} 
    Let $k \in \set{1,2,\ldots}$ and consider the operation: 
\begin{description}
    \item[Input.]  A multi-matroid $A$ together with an ordered partition $\le$ of degree at most $k$. 
    \item[Output.]  The list $[A_1,\ldots,A_n]$ of residuals of its equivalence classes. 
\end{description}
    Both this operation, and its inverse are original \mso transductions. 
\end{lemma}
\begin{proof}
    In the proof, we will use the name \emph{residual list of $(A,\le)$} for the output $[A_1,\ldots,A_n]$ of the operation. The residual list is easily seen to be definable as an \mso transduction. The interesting part is the inverse. The difficulty is that taking the residual list seems to be a lossy operation, since the list $[A_1,\ldots,A_n]$ does not store information about independence of sets that span different list elements. 
    Because of the loss of information, the inverse of the operation in the lemma is not a function, but a relation, since several different choices of $(A,\le)$ might lead to the same  residual list $[A_1,\ldots,A_n]$. Nevertheless, as we will show below, once we are given $[A_1,\ldots,A_n]$ we can use nondeterministic colouring and the logic \mso to recover all possible choices of $(A,\le)$. 

      
    For a multi-matroid, define its \emph{contextual equivalence} to be equivalent relation on subsets of elements that identifies two subsets if they belong to the same independence relations. If a multi-matroid has degree at most $k$, then its contextual equivalence has at most $2^k$ equivalence relations. 

    Let $(A,\le)$ be a multi-matroid with an ordered partition of degree at most $k$, and let $[A_1,\ldots,A_n]$ be its residual list.  We will show that the contextual equivalence of $A$ can be produced based on the residual list, using some nondeterministically guessed parameters.  Once we know the contextual equivalence of $A$, then we can recover nondeterministically all of its independence relations, since each independence relation is a union of some equivalence classes of contextual equivalence. 

    
    Define the \emph{index} of an element in the multi-matroid $A$ to be the $i \in \set{1,\ldots,n}$ such that the element belongs to $A_i$.
    For $i \in \set{1,\ldots,n}$, define $A_{\le i}$ to be the residual multi-matroid obtained from $A$ by taking the residual of the elements with index at most $i$. 
    The key property in the proof is the following compositionality principle.
\begin{claim}
    For every $i \in \set{1,\ldots,n}$ and every set $Y$ of elements in $A$, the contextual equivalence class of $Y \cap A_{\le i}$ in  $A_{\le i}$ 
    depends only on 
    \begin{itemize}
    \item the contextual equivalence class of $Y \cap A_{\le i-1}$ in $A_{\le i-1}$; and 
    \item the contextual equivalence class of $Y \cap A_i$ in $A_{i}$. 
    \end{itemize}
\end{claim}
\begin{proof}
    (TODO)
\end{proof}
Thanks to the above claim, we will be able to define a finite automaton with at most $2^k$ states, which inputs a set of elements $Y$ in $A$ (which is the same as a set of elements in $[A_1,\ldots,A_n]$), iterates along $i \in \set{1,\ldots,n}$, and each iteration computes the contextual equivalence class of $Y \cap A_{\le i}$ in $A_{\le i}$. To store the equivalence classes, the automaton will use some choice of colours that name these equivalence classes, as described below. 
For every $i \in \set{1,\ldots,n}$ choose some colouring 
\begin{align*}
\lambda_i : \powerset A_i \to 2^k
\end{align*}
such that two subsets get the same colour if and only if they are contextually equivalent in $A_i$. Likewise,  choose some colouring 
\begin{align*}
    \lambda_{\le i} : \powerset (A_{\le i}) \to 2^k
    \end{align*}
    such that two subsets get the same colour if and only if they are contextually equivalent in $A_{\le i}$. Once these colourings have been fixed, we know from the claim that for every $i \in \set{2,\ldots,n}$ there is some function 
\begin{align*}
\delta_i : 2^k \times 2^k \to 2^k
\end{align*}
such that for every set $Y$ of elements in $A$, the colour
\begin{align*}
\lambda_{\le i}(Y \cap A_{\le i})
\end{align*}
is obtained by applying $\delta_i$ to the pair of colours 
\begin{align*}
\lambda_{\le i-1}(Y \cap A_{\le i-1}) \quad \text{and} \quad \lambda_i(Y \cap A_i).
\end{align*}
In particular, once we have fixed all of the functions $\delta_2,\ldots,\delta_n$, we can recover for each set $Y$ its colour under $\lambda_{\le n}$ by using only the colours 
\begin{align*}
    \lambda_1(X \cap A_1), \ldots, \lambda_n(X \cap A_n).
\end{align*}
Finally, by definition, the colouring $\lambda_{\le n}$ gives us the contextual equivalence of $A$, and in particular it can be used to recover the multi-matroid structure, by defining each independence relation as some union of colours. Summing up, we  have described above a way to recover the multi-matroid $A$ from the input list $[A_1,\ldots,A_n]$, by using the following ingredients: 
    \begin{enumerate}
        \item for each $i \in \set{1,\ldots,n}$, a colouring $\lambda_i$ which assigns colours from $2^k$ to subsets of $A_i$ such that two subsets get the same colour if and only if they are contextually equivalent in $A_i$;
        \item  functions $\delta_2,\ldots,\delta_n$ of type $2^k \times 2^k \to 2^k$;
        \item for each independence relation in $A$, a corresponding subset of $2^k$.
    \end{enumerate}
    These ingredients can be guessed by an \mso transduction. The only non-trivial part is the colouring in the first item; this colouring can be represented by choosing for each $i \in \set{1,\ldots,n}$ and 
    each colour $c \in 2^k$ a distinguished set of elements in $A_i$, subject to the requirement that for every equivalence of class of contextual equivalence in $A_i$ there is exactly one colour $c$ that is used for subsets in that equivalence class.  

    Once we have the above ingredients, the structure of the multi-matroid $A$ can be defined in \mso. Not every choice of ingredients will give a legitimate multi-matroid, but whether or not the output is legitimate can be defined in \mso, and therefore illegitimate choices of parameters can be discarded by the \mso transduction. 
\end{proof}


By using the two mutually inverse operations from the above lemma as the encoding and decoding, we get the following corollary. 

\begin{corollary}\label{cor:equivalence-with-residual-lists}
    Let $\Cc$ be a class of multi-matroids of degree at most $k$. If $\Cc$ has  definable tree decompositions, then the same is true  for
    \begin{align*}
    \setbuild{ (A,\le)}{
        $A$ is a multi-matroid of degree at\\ most $k$, and $\le$  is an  
        ordered partition \\whose  residual list is in $\Cc^+$
    }.
    \end{align*}
\end{corollary}
\begin{proof}
    By Lemma~\ref{lem:reconstruct-multi-matroid-from-list}, the class in the conclusion of the lemma is equivalent, under  original encodings, with the class $\Cc^+$. The latter class has definable tree decompositions, because it encodes in trees$^+$, which encodes in trees.
\end{proof}




==> linear-matroid-width.tex <==
\section{Definable tree decompositions for matroids of bounded linear width}
\label{sec:appendix-definable-tree-decompositions-for-matroids}
In this part of the appendix, we prove Theorem~\ref{thm:definable-tree-decompositions-for-matroids}, which says that if a class of matroids representable over some finite field, under independence representation, has bounded linear \mso width, then it has definable tree decompositions. This is the longest proof of this paper, although it is not entirely original. It is an adapatation of the proof in~\cite[Theorem 4.1]{matroids-definability}, which shows the same result but using the stronger null representation. (When the field has two elements, these two results are the same, but they diverge for finite fields with more than two elements.) We view the value of the proof below not so much in the strength of the result (which allows a weaker matroid representation for finite fields with more than two elements), as in the use of the \mso framework that is developed in this paper. 

For the rest of this section, we fix some finite field $\field$. When we talk about reprsentable matroids, we mean those that can be represented over this field. All matroids will be given using the independence representation.


\subsection{Origins}
\label{sec:origins}
In the proof, we will be working with a finer notion of transduction, called \emph{origin semantics}~\cite{bojanczykTransducersOriginInformation2014},   which tracks the information about which elements in the output structure were created from which elements in the input struture. 

\subparagraph*{Origin semantics.}
The idea behind origin semantics is that if we apply an \mso transduction to an input structure, then we not only get an output structure, but also an implicit \emph{origin map}
which assigns to each  element of the output structure a corresponding element of the input structure that was used to create it, which is called its \emph{origin}. For example, if we consider the \mso transduction of type $2^* \to 2^*$ that duplicates the input string, the origin map looks like this: 
\mypic{10}
More generally, any \mso transduction will have some implicit origin information, which we make explicit in the following definitions. 

Define an \emph{original transduction} to be a set of triples of the form: (a) an input structure; (b) an output structure; (c) a map from the universe of the output structure to the universe of the input structure. The map in item (c) is called the \emph{origin map}. As for transductions, we require that all input structures use the same vocabulary, and all output structures use the same vocabulary, which may be different from the input vocabulary. We also require that an origin transduction is closed under isomorphisms, which means that if we take a triple in the transduction,  apply some isomorphism to the input structure, and some other isomorphism to the output structure, and modify the origin map accordingly, then the resulting triple is also in the transduction. This completes the definition of original transductions.

\subparagraph*{Origin semantics for \mso transductions.}
We will care about original transductions that can be defined \mso. The syntax for such transductions is defined in the same way as in the case without origins, only this time we observe that this syntax is also associated to origin semantics. For each \mso transduction, there is a natural way of lifting its semantics to an original transduction.
For colouring and \mso interpretations, the origin map is the inclusion map; for  the copying transductions, all  copies of an element have that element as its origin. Finally, original transductions are composed in the natural way, using the composition of the two origin maps. Since original \mso transductions are closed under composition, they also form a category; this category admits a forgetful functor to the category of (non-original) \mso transductions by forgetting the origins. 



\begin{definition}[Original encoding]
    An \emph{original encoding} is an original \mso transduction that admits a one-sided inverse, i.e.~there is an original \mso transduction, which we call \emph{decoding}, 
    \[
    \begin{tikzcd}
    \Cc 
    \ar[r,"encode", bend left=20] &
    \Dd
    \ar[l,"decode", bend left=20] 
    \end{tikzcd}
    \]
    such that encode followed by decode contains the (origin) identity on $\Cc$. 
\end{definition}

% \newcommand{\vleq}{\mathrel{\rotatebox{90}{$\le$}}}


In general, this notion of encoding is incomparable with the \mso encodings from Definition~\ref{def:mso-encoding}. The difference can be seen in the  degenerate case when both classes $\Cc$ and $\Dd$ are finite up to isomorphism. In this case, the two kinds of encodings can be characterized as follows: there is a (non-original) \mso encoding from $\Cc$ to $\Dd$ if and only if 
\begin{align}
    \label{eq:number-of-isomorphism-types}
    \begin{tabular}{c}
        number of isomorphism types in $\Cc$
        \\
        $\vleq$\\
        number of isomorphism types in $\Dd$,
    \end{tabular}
\end{align} 
while an original encoding from $\Cc$ to $\Dd$ exists if and only if 
\begin{align}
    \label{eq:maximal-universe-size}
\begin{tabular}{c}
    maximal universe size in $\Cc$ \\
    $\vleq$\\
    maximal universe size in $\Dd$.
\end{tabular}
\end{align} 
Since conditions~\eqref{eq:number-of-isomorphism-types} and~\eqref{eq:maximal-universe-size} are incomparable, so are the corresponding encodings. However, when the class $\Dd$ is the class of all trees, which is the case of interest in this section, then original encodings are a stronger notion than \mso encoding, as explained in the following lemma. 


\begin{lemma}\label{lem:original-to-trees-non-original} If a class of structures  admits  an original encoding from $\Cc$ to trees, then it also admits  a (non-original) \mso encoding  to trees.
\end{lemma}
\begin{proof} We prove a slightly more general result, namely the lemma holds even if the class of trees is replaced by any class $\Dd$ that satisfies a certain assumption, which we call \emph{encoding colourings}, that will be explained later in the proof. Under this assumption, original encodings are also equivalent to a stronger notion: define  a \emph{strong original encoding} in the same way as an original encoding, except that we require that encode;decode is equal to the identity, and not just contains it. The following diagram explains the  relationships between the three kinds of encodings:
    \[
    \begin{tikzcd}
    \text{there is an original encoding from $\Cc$ to $\Dd$} 
    \ar[d,Rightarrow,shift left=2, "{\text{if $\Dd$ can encode colours}}"] 
    \\
    \text{there is a strong original encoding from $\Cc$ to $\Dd$} 
    \ar[d,Rightarrow, "{\text{without any assumptions on $\Dd$}}"] 
    \ar[u,Rightarrow,shift left=2,"{\text{without any assumptions on $\Dd$}}"] 
    \\
    \text{there is a \mso encoding from $\Cc$ to $\Dd$} 
    \end{tikzcd}
    \]
    The implications in the above diagram that do not use any assumptions are immediate consequences of the definitions. The assumption on encoding colours is necessary for the remaining implication, which can be shown using finite classes of structures. 

    It remains to  define  the assumption on encoding colours, prove that the class of trees satisfies it, and to prove the implication in the diagram that uses this assumption. The lemma will follow by composing the two downward implications in the diagram. 
 
    For a class of structures $\Dd$, define \emph{$k$-coloured $\Dd$} to be the class of structures obtained from $\Dd$ by applying $k$-colouring. For example, $k$-coloured trees is the class of trees with a nodes labelled by $k$ colours. 
We say that a class of structures \emph{encodes colours} if for every $k \in \set{1,2,\ldots}$, the class is equivalent, under strong under original encodings, with its $k$-coloured version. 
Encoding colours seems to be a mild assumption. For example, the class of trees encodes colours, which follows using the encoding given in Lemma~\ref{lem:other-unordered-trees}. In fact, all classes of structures discussed in Theorem~\ref{thm:figure-encodings} encode colours, except for the trees of bounded height.  

To complete the proof of the lemma, it remains to show that  if $\Dd$ encodes colours, and there is an original encoding from $\Cc$ to $\Dd$, then there is also a strong original encoding. This will follow immediately from the following claim, and the fact that strong original encodings are closed under composition. 

\begin{claim}
    If there is an original encoding from $\Cc$ to $\Dd$, then for some $k$ there is a strong original encoding from $\Cc$ to $k$-coloured $\Dd$. 
\end{claim}
\begin{proof}
    By assumption, we have two original \mso transductions 
    \[
        \begin{tikzcd}
        \Cc 
        \ar[r,"\text{encode}", bend left=20] &
        \Dd
        \ar[l,"\text{decode}", bend left=20] 
        \end{tikzcd}
        \]
    such that encoding followed by decoding is an original \mso transduction from $\Cc$ to itself which contains the identity.  Our goal is to improve these transductions so that encoding followed by decoding is equal to the identity.      Like any original \mso transduction, the decoding from $\Dd$ to $\Cc$ is the composition of colouring with some deterministic transduction. If we integrate the colouring into the encoding, and then in the encoding we push the colouring to the beginning, we see that there is some $k \in \set{1,2,\ldots}$ and  some deterministic original transductions $f$ and $g$, as in the following diagram
        \[
        \begin{tikzcd}
        & \text{$k$-coloured $\Cc$}
        \ar[dr,"f"]
        \\
        \Cc 
        \ar[ur,"\text{$k$-colouring}", ]
         & &
        \text{$k$-coloured }\Dd
        \ar[ll,"g"] 
        \end{tikzcd}
        \]
    such that starting in $\Cc$ and taking one cycle in the diagram gives a superset of the identity on $\Cc$. We now want to make that superset to be equal to the identity. For each structure $A \in \Cc$, we can consider two kinds of $k$-colourings: the good colourings are those such that $f;g$ applied to them returns to the original structure $A$, and the bad colourings are the remaining ones. One can write an \mso formula which inputs a structure in $k$-coloured $\Cc$ and tells us if the colouring is good (the use of origin semantics is crucial here, otherwise the \mso formula would need to decide isomorphism on structures). We can now modify $f$ by reducing its domain to good colourings; as a result we get a strong original encoding. 
\end{proof}

The above claim completes the proof of the lemma.
\end{proof}



In the rest of this section, we will be working with (not necessarily strong) original encodings. We will prove that if a class of structures has bounded linear \mso width, then it admits an original encoding to trees. We use the following name for such classes. 

\begin{definition}[Original tree decompositions] \label{def:original-tree-decompositions}
    We say that a class of structures $\Cc$ has \emph{definable tree decompositions} if it admits an original encoding to trees. 
\end{definition}

By Lemma~\ref{lem:original-to-trees-non-original}, if a class has original tree decompositions, then it has definable tree decomositions as in Definition~\ref{def:definable-tree-decompositions}. In the rest of this  section, we will show that if $\Cc$ is a class of representable matroids over some finite field, and $\Cc$ has linear \mso width, then it has original tree decompositions. This will imply Theorem~\ref{thm:definable-tree-decompositions-for-matroids}. 





\input{operations-dtd}
\input{ap-hom-ord-part}
\input{defining-linear-orders}
\input{simon}

==> operations-dtd.tex <==
\subsection{Original tree decompositions for matroid minors}
In the proof that representable matroids of bounded linear \mso width have original tree decompositions, we will use several operations on multi-matroids that preserve original tree decompositions. Examples of such operations include classic matroid operations such as deletions, contractions and taking connected components, but we also describe other operations that are specific to the setting of multi-matroids.

\begin{enumerate}
    \item \textbf{Dual.} The \emph{dual} of a matroid $A$ is the matroid, denoted by $A^*$, which has the same ground set, and in which the matroid structure is defined by 
    \begin{align*}
    X \text{ is a basis of } A^* \qquad \iff \qquad \text{complement of $X$ is a basis of $A$}.
    \end{align*}
    \item \textbf{Deletion.}      
    The \emph{deletion} operation for a matroid is defined as follows. If $X$ is a set of elements in a matroid $A$, then $A\setminus X$ is the matroid in which the elements are the complement of $X$, and the independent sets are inherited from $A$ (restricted to the smaller set). 
    \item \textbf{Contraction.} 
    The \emph{contraction} operation for a matroid is defined as follows. If $X$ is a set of elements in a matroid $A$, then the contracted matroid $A/X$ is defined dually to deletion as follows:
    \begin{align*}
    A / X = (A^* \setminus X)^*.
    \end{align*}
    An alternative, but equivalent, definition is as follows. Choose some maximal independent set $Y \subseteq X$ contained in $X$. In the contracted matroid $A/X$, the elements are those that are not in $X$, and the independent subsets are those which remain independent after adding $Y$.  This definition does not depend on the choice of $Y$, and it is equivalent to the one by duality with deletion. 
\end{enumerate}

    The above operations make sense for general matroids. One can show that contractions and deltions commute, i.e.
    \begin{align*}
        A\setminus x / y = A / y \setminus x,
    \end{align*}
    and therefore one need not specify the order of operations when contracting and deleting multiple elements.    A matroid obtaind from $A$ by deleting some elements and contracting some other elements is called a \emph{minor} of $A$. If a  is matroid representable over our fixed field, then the same is true for all of its minors.

    The following lemma  shows that original tree decompositions are not affected when deleting an element. In the lemma we use the assumption that the matroids are representable over a fixed field.

\begin{lemma}\label{lem:decontract}
 If a class of matroids $\Cc$ over a fixed finite field $\field$  has original tree decompositions, then the same is true for 
 \begin{align*}
\setbuild{A}{$\Cc$ contains $A\setminus x$ for some element $x$ of $A$}.
 \end{align*}
\end{lemma}
Since contractions are dual to deletions, and taking the dual is an isomorphism in our category, it follows that  Lemma~\ref{lem:decontract} also holds when instead of deletions we use contractions. By applying the above lemma and its dual for contractions several times, we get the following corollary. 
\begin{corollary}\label{cor:minor-dtd}
    Let $\Cc$ be a class of matroids, and let $\ell \in \set{1,2,\ldots}$. If $\Cc$ has original tree decompositions, then the same is true for 
 \begin{align*}
\setbuild{A}{$\Cc$ contains the $A\setminus X_1 / X_2$ for some disjoint sets $X_1,X_2$ such that $|X_1 \cup X_2| \le \ell$}.
 \end{align*}
\end{corollary}


% \begin{proof}
% To prove the equivalence in the lemma, we will proceed in several steps.  Contracting a set $\set{x_1,\ldots,x_m}$ can be done in several steps: we can first contract $x_1$ (formally speaking, contract the singleton set $\set {x_1}$), then contract $x_2$, and so on until $x_n$. The result of this multi-step procedure is the same as contracting the entire set in a single step. This proves that 
%  \begin{align*}
%  \Cc/(m_1 + m_2) = (\Cc/m_1)/m_2.
%  \end{align*}
%  Therefore, it is enough to prove the lemma for $m=1$.


% Observe that an element of a matroid (or multi-matroid) could be dependent even in isolation from other elements. (In a matroid which arises from a vector space, this happens when the element represents the zero vector.)
%  For a multi-matroid with $k$ independence relations, define the \emph{independence type} of an element $x$ to be the set 
%  \begin{align*}
%  \setbuild{i \in \set{1,\ldots,k}}{$\set{x}$ is in the $i$-th independence relation}.
%  \end{align*}
%  The definition of an independence type assumes that the independence relations have numbers in $\set{1,\ldots,k}$, which is the case for multi-matroids represented as structures. 
%  For a set $I \subseteq \set{1,\ldots,k}$ define $\Cc_I$ to be the class of multi-matroids that can be obtained by taking some multi-matroid in $\Cc$ and contracting a single element of independence type $I$. By definition we have 
%  \begin{align*}
%  \Cc/1 = \bigcup_{I \subseteq \set{1,\ldots,k}} \Cc_I.
%  \end{align*}
%  Since having original tree decompositions is closed under subsets and finite unions, the above class has original tree decompositions if and only if $\Cc_I$ has original tree decompositions for every $I \subseteq \set{1,\ldots,k}$. Since having original tree decompositions is also closed under finite co-products, it follows that $\Cc/1$ has original tree decompositions if and only if the same is true for 
%  \begin{align}\label{eq:typed-contractions}
%  \coprod_{I \subseteq \set{1,\ldots,k}} \Cc_I.
%  \end{align}
%  For reasons which will be explained in Footnote~\ref{footnote:why-adjoin}, we modify the above class slightly, by adjoining a fresh element to each structure. More precisely, let $1$ be the class of structures which contains exactly one structure that has one element in its universe and no relations. If $\Dd$ is a class of structures, then $1 \times \Dd$ is the class of structures that arise from structures in $\Dd$ by adjoining a fresh distinguished element, which is not related with any element of $\Dd$. It is easy to see that this operation does not affect having original tree decompositions, i.e.~$\Dd$ has original tree decompositions if and only if the same is true for $1 \times \Dd$. Therefore, the class in~\eqref{eq:typed-contractions} has original tree decompositions if and only if the same is true for 
%  \begin{align}\label{eq:typed-contractions-adjoined}
%  \coprod_{I \subseteq \set{1,\ldots,k}} 1 \times \Cc_I.
%  \end{align}
%  To complete the proof, we will show that the above class is isomorphic to $\Cc$, under \mso transductions with origin\footnote{\label{footnote:why-adjoin} If we wanted isomorphism without origins, we could have used the class~\eqref{eq:typed-contractions}. However, the notion of original tree decompositions from Definition~\ref{def:definable-tree-decompositions} requires the encoding to take into account origins, which is why adjoint the extra element, so that it can be used as the origin of the contracted element.}. The isomorphism from $\Cc$ to the class~\eqref{eq:typed-contractions-adjoined} picks an element, contracts it, and puts the result in the component of the co-product that corresponds to the independence type of the element. This operation is easily seen to be definable in \mso, and the same is true for its inverse. 
% \end{proof}

% In the following lemma, we will consider the opposite process of contraction, which can be called \emph{de-contraction}, i.e.~multi-matroids which admit some contraction in $\Cc$:
 

% \begin{lemma}\label{lem:decontract-elements}
%  Let $\Cc$ be a class of multi-matroids of degree at most $k$. Then $\Cc$ has original tree decompositions if and only if the same is true for
%  \begin{align*}
%  \setbuild{A}{$A/x \in \Cc$ for some $x \in A$}.
%  \end{align*}
%  \end{lemma}
% \begin{proof}
%     (TODO)
% \end{proof}

% In many situations, it will be more convenient to specify the residual not by describing the elements which are removed, but rather the elements that stay, as in the following notation:
% \begin{align*}
% \multimata  @ X \eqdef \multimata \div \text{(complement of $X$)}.
% \end{align*}
% In other words, the residual $\multimata @ X$ is the family of matroids that can be obtained by taking a minor with elements $X$ of some matroid in the family $\multimata$.



==> rubbish.tex <==


% We only desribe the second \mso encoding. Consider a hypergraph $G$. Its \emph{plot hypergraph} is defined as follows. For every vertex in $G$, there are two copies in the plot hypergraph, called the ``yes'' and ``no'' copies. For every hyperedge, in $G$, there is a hyperedge in the plot graph of the form 
% \begin{align*}
% \setbuild{\text{``yes'' copy of $v$}}{$v \in X$} \cup 
% \setbuild{\text{``no'' copy of $v$}}{$v \not \in X$}.
% \end{align*}
% Here is a picture of this construction:
% \mypic{22}


% For a hyperegraph, define its \emph{downward closure} to be the hyperegraph with the same vertices, but where the hyperedges are the original hyperedges and their subsets. A hypergraph is called \emph{downward closed} if it is its own downward closure.
% \begin{claim}
% If a hypergraph $G$ is downward closed, then the downward closure of its plot hypergraph is a matroid.
% \end{claim}
% \begin{proof} We will show that the hyperedges in the plot hypergraph are \emph{bases} of some matroid, i.e.~maximal independent sets. This will mean that the downward closure of the plot hypergraph is a matroid.
 
% If a matroid is given by bases, then the independence axiom becomes: for every two different bases $B_1$ and $B_2$, there is some element $b \in B_1 \setminus B_2$ such that 
% We claim that if a hypergraph is downard closes, then its plot hypergraph is a matroid in basis representation. To prove this consider two hyperedges in the plot hypergraph, that arise from two different hyperedges $X_1$ and $X_2$ in the original hypergraph $G$. Since these two hyperedges are different, there must be some vertex $x$ of the original hypergraph that belongs to one but not the other, say $x$ belongs to $X_1$ but not to $X_2$. Since the original hypergraph is downard closed, we know that $X_1 \setminus \set x$ is a hyperedge of the original hypergraph. The corresponding hyperedge in the plot hypergraph is obtained by taking the hyperedge corresponding to $X_1$, and changing the copy of $x$ from the ``yes'' copy to the ``no'' copy. This proves the basis exchange axiom, since the ``no'' copy belongs to the hyperedge that corresponds to $X_2$.
% \end{proof}
 
% \begin{claim}
% If a hypergraph is downward closed, then $M(G)$ is a matroid.
% \end{claim}
% \begin{proof}
% Consider two independent sets $I_1$ and $I_2$ in the encoding. By definition, we have 
% \begin{align*}
% I_1 \subseteq \bar{X_1} \quad I_2 \subseteq \bar{X_2}
% \end{align*}
% for some hyperedges $X_1$ and $X_2$ in the hypergraph. If 
% \end{proof}
% \end{proof}

The right-to-left encodings in the first line are simply inclusions. The encoding of hypergraphs in downward closed ones is a left to the reader. Below we explain the encodings of downward closed hypergraphs in uniform ones, and the encoding of uniform hypergraphs in general matroids.  
    
\subparagraph*{From downard closed  hypergraphs to uniform hypergraphs.} Consider a downward closed hypergraph $G$. Its \emph{plot hypergraph},  is defined as follows. For every vertex in $G$, there are two copies in the plot hypergraph, called the ``yes'' and ``no'' copies. For every hyperedge, in $G$, there is a hyperedge in the plot graph of the form 
    \begin{align*}
    \setbuild{\text{``yes'' copy of $v$}}{$v \in X$} \cup 
    \setbuild{\text{``no'' copy of $v$}}{$v \not \in X$}.
    \end{align*}
By definition, the plot hypergraph is uniform, since all hyperedges have the same size, namely the number of vertices in the original hypergraph.
    Here is a picture of this construction:
    \mypic{22}
The construction of the plot hypergraph does not use the assumption that the input hypergraph is downward closed. This assumption will be used in the decoding. The purpose of this assumption is to recover the matching between vertices of the plot hypergraph, which assigns to each ``yes'' copy the corresponding ``no'' copy. This correspondence is obtained as follows We say that a vertex $y$ is a \emph{shadow} of a vertex $x$ if for every hyperedge that contains $x$, replacing $x$ with $y$ gives another hyperedge. One can show that in the plot hyperegraph obtained from a downward closed hypergraph, the shadow relation is the matching that assigns to each ``yes'' copy the corresponding ``no'' copy. The decoding uses this shadow relation to revover the original hypergraph.


We assume that $\alpha$ is a linear \mso interpretation, i.e.~there is no colouring or copying. This is because the colours and the copies can be integrated into the input string. This means that there are 
\begin{align*}
\myunderbrace{h : (\Sigma \times 2)^* \to A}{monoid homomorphism \\ \scriptsize with $A$ finite} \qquad \myunderbrace{\elemset, \nullset : A \to \set{\text{yes, no}}}{distinguished subsets}
\end{align*}
such 
the  elements and null sets  of the output matroid $\alpha(w)$ are 
\begin{eqnarray*}
&&\setbuild{ x }{$x$ is a position in $w$ such that $h(w \otimes \set x) \in \text{elem}$}\\
  &&  \setbuild{ X }{$x$ is a set of  positions in $w$ such that $h(w \otimes \set X) \in \text{null}$}.
    \end{eqnarray*}
We assume that the homomorphism is surjective and  minimal in the  sense that the following equivalence relation on $A$ has only singleton equivalence classes
\begin{align*}
a \sim a' \qquad \eqdef \qquad  \forall b,c \in A \ \land \begin{cases}
    bac \in \elemset \iff ba'c \in \elemset\\
    bac \in \nullset \iff ba'c \in \nullset.
\end{cases}
\end{align*}
This assumption can be made without loss of generality, by restricting the homomorphism to its image and quotienting the image by $\sim$. 


For $u,v \in \Sigma^*$, define an \mso string-to-matroid transduction 
\begin{align*}
u\alpha v : \Sigma^* \to \text{matroids}
\end{align*}
as follows: use the same homomorphism $h$, but replace the  accepting sets $\elemset$ and $\nullset$  with 
\begin{align*}
\setbuild{a \in A} { $h(u \otimes \emptyset) \cdot a \cdot h(v \otimes \emptyset) \in \elemset$ }\\
\setbuild{a \in A} { $h(u \otimes \emptyset) \cdot a \cdot h(v \otimes \emptyset) \in \nullset$ }
\end{align*}
Any function of the form $u \alpha v$ is called a \emph{derivative} of $\alpha$. There are finitely many derivatives, since the derivative depends only on the images under $h$ of $u \otimes \emptyset$ and $v \otimes \emptyset$. 
We say that a set $L \subseteq \Sigma^*$ is \emph{simple} if 
\begin{align*}
\bigcup_{\alpha '} \alpha'(L)
\end{align*}
has definable tree decompositions, where $\alpha'$ ranges over derivatives of $\alpha$. 
\begin{lemma}
    Simple subsets of $\Sigma^*$ are closed under union $L_1 \cup L_2$ and concatenation $L_1 \cdot L_2$. 
\end{lemma}
\begin{proof}
    The only interesting case is concatenation. Consider 

\end{proof}
Consider a monoid homomorphism
\begin{align*}
g : \Sigma^* \to B,
\end{align*}
which will be chosen later on. Define the Simon height of a word $w \in \Sigma^*$, with respect to $g$, as follows: 


Consider a matroid of the form 
\begin{align*}
M = \alpha(w_1 \cdots w_n)
\end{align*}
such that $w_1,\ldots,w_n$ have the same idempotent image $e$ under $g$, and Simon height at most $k$. Let $X$ be the elements of $M$, this set can be seen a subset of the positions in $w$, and consider the partition 
\begin{align*}
X = X_1 \cup \cdots \cup X_n
\end{align*}
where $X_i$ is the positions from $X$ that are in $w_i$. 
Let  $V$ be the vector space of this matroid, i.e.~the quotient of the vector space $2^X$ by the nulls. Define the \emph{representation} to be the function of type $2^X \to V$ which quotients a vector under the nulls.  For $i \in \set{1,\ldots,n}$, define $V_i$ to be the subspace of $V$ which consists of  representations of subsets of $X_i$. 

\begin{lemma}\label{lem:interfaces}
    For every $i \in \set{1,\ldots,n}$ the number of vectors in   
    \begin{align}\label{eq:vectors-on-two-sides}
    \vecspan {V_1 \cup \cdots \cup V_i} \cap \vecspan{V_{i+1} \cup \cdots \cup V_n}
    \end{align}
    is at most the size of the monoid $A$. Furthermore, 
    \begin{align}\label{eq:gap-inclusion}
        \vecspan {V_1 \cup \cdots \cup V_{i-1}} \cap \vecspan{V_{i+1} \cup \cdots \cup V_n} \subseteq \myunderbrace{V_1 \cap V_n}{call this $U$}
        \end{align}
\end{lemma}
\begin{proof}Let us first show that the number of vectors in~\eqref{eq:vectors-on-two-sides} is at most the size of the monoid. Here we do not need any assumptions on $w_1,\ldots,w_n$ having the same image. In fact, we prove  a stronger result: namely for every words $u_1,u_2$, the following vector space has at most one vector per element of $A$:
    \begin{align}\label{eq:two-sides-of-u1-u2}
    \bigcap_{i \in \set{1,2}}\setbuild{\text{representation of $X_i$ in $\alpha(u_1u_2)$}}{$X_i$ is a set of positions in $u_i$}.
    \end{align}
    From this we get the statement of the lemma, by setting $u_1 = w_1 \cdots w_i$ and $u_2 = w_{i+1} \cdots w_n$. To see why the intersection~\eqref{eq:two-sides-of-u1-u2} is small, consider a vector in this intersection, as witnessed by two sets $X_1$ and $X_2$, one contained in $u_1$ and one contained in $u_2$.  Suppose now that  $Y_1$ is a set  of positions in $u_1$  such that 
    \begin{align*}
    h(u_1 \otimes Y_1) = h(u_1 \otimes X_1).
    \end{align*}
    Because $h$ tells us which sets are null, and $X_1 \cup X_2$ is null because the sets $X_1$ and $X_2$ represent the same vector, we know also that $Y_1 \cup X_2$ is null. This means that $Y_1$ must represent the same vector as $X_1$. Summing up, every vector in the intersection~\eqref{eq:two-sides-of-u1-u2} is uniquely determined by the image $h(u_1 \otimes X_1)$, and the number of such images is at most the size of $A$. 

    Consider now the inclusion~\eqref{eq:gap-inclusion}. 
    A vector on the left side of the inclusion can be represented as two sets:
    \begin{align*}
    Y_1 \cup \cdots \cup Y_{i-1} \qquad Y_{i+1} \cup \cdots \cup Y_n,
    \end{align*}
    such $Y_j \subseteq X_j$ for every $j$.
    By assumption on the images of $w_1,\ldots,w_n$ all being idempotent, we know that $w_1$ has the same image as $w_1 \cdots w_{i-1}$. This means that one can find a set $Z_1 \subseteq X_1$ such that 
    \begin{align*}
        h(w_1 \otimes Z_1) = h((w_1 \otimes Y_1) \cdots (w_{i-1} \otimes Y_{i-1}))
        \end{align*} 
Since $w_i$ has the same image as $w_{2} \cdots w_{n-1}$, we know that 
    \begin{align*}
    h(w_i \otimes \emptyset) = h((w_2 \otimes \emptyset) \cdots (w_{n-1} \otimes \emptyset)).
    \end{align*}
    Putting these two equalities together, we see that 
    \begin{align*}
    h((w_1 \cdots w_i) \otimes (Y_1 \cup \cdots \cup Y_{i-1})) = h((w_1 \cdots w_i) \otimes Z_1),
    \end{align*}
    and therefore the sets  $Y_1 \cup \cdots Y_{i-1}$ and $Z_1$ represent the same vector.  For similar reasons, we can find a set $Z_n$ of positions in $w_n$ such that   the sets $Y_{i+1} \cup \cdots \cup Y_n$ and $Z_n$ represent the same vector, which completes the proof of the lemma. 
\end{proof}

Define $U = V_1 \cap V_n$. A set of elements $X$ in $\alpha(w)$ is called a \emph{$U$-circuit} if it is a minimal inclusionwise set in the family 
\begin{align*}
\setbuild { Y } { $Y$ is nonempty set of elements in $\alpha(w)$ that  represents a vector in $U$}.
\end{align*}
This is the same thing as being a circuit, in the usual matroid sense, in the matroid obtained from $\alpha(w)$ by contracting the subspace $U$. Let $x \sim y$  be the equivalence relation on elements of $\alpha(w)$ which holds if $x=y$ or there is some $U$-circuit that contains both $x$ and $y$. 

\begin{lemma}
    Let $w_1,\ldots,w_n \in \Sigma^*$ be words with the same type, which is idempotent. 
    Define the \emph{index} of an element in $\alpha(w_1 \cdots w_n)$ to be the unique $i$ such that the element comes from $w_i$, and define the \emph{colour} of an element to be its index modulo 5.  For every every $\delta \in \set{0,1}$ and every two elements $x,y$ in $\alpha(w)$, the following conditions are equivalent:
    \begin{enumerate}
        \item $index(y) = index(x) + \delta$ and there is a $U$-circuit that contains $x$ and $y$;
        \item $colour(y) = colour(x)+ \delta$ and there is a $U$-circuit that contains $x$ and $y$ but uses at most 4 colours. 
    \end{enumerate}
\end{lemma}
\begin{proof}\ 
    \begin{itemize}
        \item[2$\Rightarrow$1] Let $i,j$ be the indices of $x$ and $y$, and let $C$ be a circuit that connects $x$ and $y$ and uses at most 4 colours. This circuit witnesses the circuit part of item 1, and it remains to prove that $j = i+\delta$.
            Let $I$ be the indices used by the circuit $C$. By the ``Furthermore'' part of  Lemma~\ref{lem:interfaces},  $I$ must contain the interval between $i$ and $j$, i.e.~$I$ must contain every $\ell$  with 
            \begin{align*}
            \min(i,j) \le \ell \le \max(i,j)
            \end{align*}
             since  otherwise intersecting $C$ with positions of index $< \ell$ would give a nonempty proper subset of $C$ that represents a vector in $U$.  Since $I$ has at most four colours, it follows that $|i-j| \le 3$. This, in conjunction with the colour constraint from item 2, implies that $j=i+\delta$. 
        \item[1$\Rightarrow$2] Let $i$ be the index of $x$.  Clearly if the index of $y$ is $\delta+i$,  then the same relationship holds modulo 5. Let us now find a circuit that connects $x$ and $y$, and avoids some colour. We will prove that there is a circuit that connects $x$ and $y$, and uses positions with at most 4 indices (and therefore at most 4 colours).  We know that there is a circuit $C$ that connects $x$ and $y$. This means that $w \otimes C$ belongs to the circuit language. Decompose $w$ into three parts 
        \begin{align*}
            w  = 
            \myunderbrace{w_1 \cdots w_{i-1}}{left}
            \myunderbrace{w_i \cdots w_{i+\delta}}{middle}
            \myunderbrace{w_{i+\delta+1} \cdots w_{n}}{right}.
            \end{align*}
        Likewise we factorize $w \otimes C$ into three parts, and partition circuit $C$ into three parts.  Since the left part of $w$  has the same image under the powerset of the circuit homomorphism as $w_{i-1}$, we know that there is  a set $D_{\text{left}}$ of positions in $w_{i-1}$ such that $w_{i-1} \otimes D_{\text{left}}$ has same image under the circuit homomorphism as the left part of $w \otimes C$. A similar thing can be done for the right part, yielding a set of positions $D_{\text{right}}$ in $w_{i+\delta+1}$. Summing up, the set 
            \begin{align*}
            D = D_{\text{left}} \cup \text{(middle part of $C$)} \cup D_{\text{right}},
            \end{align*}
            is a circuit, because  $(w_{i-1}\cdots w_{i+\delta+1}) \otimes D$ has same image under the circuit homomorphism as $w \otimes C$.  Since $D$ uses at most four indices (and therefore at most four colours), and it contains the middle part of $C$ which contains both $x$ and $y$,  we obtain condition 2.        
    \end{itemize}
\end{proof}




\begin{lemma}
    There is an invertible matroid-to-tree transduction $\beta$ which is defined on every matroid of the form 
    \begin{align*}
    \alpha(w_1 \cdots w_n) \cap X
    \end{align*}
    where $w_1,\ldots,w_n$ are words with the same idempotent type, and $X$ is an inner component.
\end{lemma}
\begin{proof}
    Take a matroid as in the assumption of the lemma, and let $X_i$ be the set $X$ intersected with positions from $w_i$. Define $M_i$ 
\end{proof}
For a $Y \in \Yy$, define 
A set $X$ is null in $M$ if and only if 
\begin{lemma}
    For a component $Y$ of $M$, consider the partial function 
\begin{align*}
f_Y : \powerset Y \to U,
\end{align*}
which maps a subset of $Y$ to the vector that it represents, but with its domain restricted to subsets that represent vectors in $U$. A set of elements $M$ in $X$ is null if and only if all of the vectors 
\begin{align*}
0 = \sum_{Y}  f_Y(X \cap Y)
\end{align*}

\end{lemma}

When is a subset $X$ null? This happens if for every $Y$ which is a $U$-component. 
\begin{align*}
\text{$X$ is null in $M$}\qquad\text{iff}\qquad 
0 = 
\end{align*}

Fix $U$ as in the above lemma. For each $a \in A$, choose a set $X_{1,a} \subseteq X_1$ such that  
\begin{align*}
h(w_1 \otimes X_{1,a}) = a,
\end{align*}
if there is no such set then define $X_{1,a}$ to be empty. Consider a word 
\begin{align*}
v \in (\Sigma \times 2^A \times 2^5)^*
\end{align*}
 For each vector $v \in U$ choose a set of elements that represents it, and also 
Define a \emph{separator} to be a set $Y \subseteq X$ such that every set $Z \subseteq X$ satisfies  
\begin{align*}
\vecrep(Z) \in U \qquad \text{implies} \qquad \vecrep(Z \cap Y) \in U.
\end{align*}
(This is the usual notion of separators in a binary matroid, using the quotient binary matroid $2^X \to V/U$. )
It is easy to see that if $Y$ is a separator then the same is true for its complement $X - Y$, and also the family of separators is closed under intersection. By closure under intersection, each separator is partitions uniquely into minimal nonempty separators; the minimal nonempty separators are called \emph{components}. 

\begin{lemma} Define a partial order $x \le y$ on elements of $X$ which holds if $x$ and $y$ are connected and the index of $y$ is greater or equal to the index of $x$.  There exists an \mso formula $\varphi(x,y)$, over an input alphabet $\Sigma \times \Gamma$, such that 
    for every  $w = w_1 \cdots w_n$ there is a
    \begin{align*} 
  \exists v \in \Gamma^* \ \forall x, y \qquad     x \le y  \quad \iff \quad w \otimes v \models \varphi(x,y)
    \end{align*}
    Then $x \le y$ is defined in $v$ by an \mso  formula that depends only on ...
\end{lemma}
 


Let $Y$ be a component of $X$. By induction assumption, there is a matroid-to-tree section that is defined on every matroid of the form $M \cap (Y_i \cap X)$. We first show that there is a matroid-to-tree section that is defined on


The tree looks as follows. For a component $Y$ of $X$, define a tree $T_Y$ is 
    
For $k \in \set{0,1,\ldots}$, define a $k$-ported graph to be a graph together  with a sequence of $k$ distinguished vertices, called ports. All ports must be different.  We view graphs with ports as a multi-sorted algebra, in which for every $k \in \set{0,1,\ldots}$ there is a sort for graphs with $k$ ports, and which has the following operations: 
\begin{enumerate}
    \item \textbf{Constants.} Every $k$-ported graph is a constant, in sort $k$.
    \item \textbf{Renaming ports.} Consider any function  
\begin{align*}
    \alpha : \set{1,\ldots,\ell} \to \set{1,\ldots,k} \qquad \text{with }\ell, k \in \set{0,1,\ldots}.
\end{align*}
This function yields an operation of type 
\begin{align*}
\text{$k$-ported graphs} \to \text{$\ell$-ported graphs}
\end{align*}
defined as follows: the graph  is not changed, and the $i$-th  port in the output is the $\alpha(i)$-th port of the input.
\item \textbf{Fusion.} For every $k \in \set{0,1,\ldots,}$ there is a fusion operation of type 
\begin{align*}
    \text{($k$-ported graphs)} \times     \text{($k$-ported graphs)} \to \text{$k$-ported graphs}
    \end{align*}
which is explained in the following picture: 
\end{enumerate}

Define the \emph{\textsc{hr}-algebra} to be the multi-sorted algebra, which has one sort for each $k \in \set{0,1,\ldots}$, representing $k$-ported graphs, and which is equipped with the operations described above. 
Define a \emph{congruence} in this algebra to be any equivalence relation on its elements, which identifies only elements of the same sort, and which is compatible with all operations in the algebra in the usual sense. A language of graphs is called \emph{\textsc{hr}-recognizable} if there is a congruence such that: (a) in each sort there are finitely many equivalence classes; and (b) the language is a union of equivalence classes. The union in item (b) is necessarily finite, since the language lives in sort $k=0$, which has finitely many equivalence classes by item (a). 

The following theorem shows that \hr-recognizability coincides to our abstract notion of recognizability, using the incidence representation of graphs. 

\begin{theorem}
    A language of graphs is \textsc{hr}-recognizable if and only if 
    \begin{align*}
    \text{incidence representations of $L$}
    \quad \subseteq \quad 
    \text{incidence representations of graphs}
    \end{align*}
     is recognizable in the sense of Definition~\ref{def:recognizability}.
\end{theorem}
\begin{proof}
    We begin with the left-to-right implication. Suppose that $L$ is a language of graphs that is \hr-recognizable. Consider some function 
    \begin{align*}
    f : \text{trees} \to \text{incidence representations of graphs}
    \end{align*}
    which is an \mso transduction. 
     We will use trees with nodes labelled by operations of the \hr-algebra to represent terms in this algebra. For general multi-sorted algebras the trees would need to be ordered, but the order will not be needed for the \hr-algebra thanks to the following property 
     \begin{itemize}
        \item[$\heartsuit$] Every operation has either at most one argument, or  it is multiset operation. Here an multiset operation is an operation that has two inputs, both inputs the same sort which also equal to the output sort, and it satisfies 
        \begin{align*}
        \myunderbrace{f(a,b) = f(b,a)}{commutative} \qquad 
        \myunderbrace{f(a,f(b,c)) = f(f(a,b),c)}{associative}.
        \end{align*}
     \end{itemize}
     A multiset operation can be applied to a multiset of arguments in the natural way, and the outcome does not depend on the order of application thanks to the associativity and commutativity axioms. Thanks to property $\heartsuit$, a term in \hr-algebra can be seen as an unordered tree, since the non-binary operations can be applied to unordered multisets of arguments. For a tree with nodes labelled by operations, its value is the element of the \hr-algebra that is defined in the natural way. The value may be undefined, if the terms is ill-typed, i.e.~for some node, one of its children produces a value whose type does not match the input type of the operation 
     
     

\begin{lemma}
    For every functional \mso transduction 
    \begin{align*}
        f : \text{trees} \to \text{incidence representations of graphs}
        \end{align*}
    one can find a finite set of operations $\Gamma$ in the \hr-algebra, and an \mso transduction $h$ which makes the following diagram commute 
\end{lemma}
    By the proof of Theorem~\ref{thm:courcelle-engelfriet-width-logical}, one can find a finite set $\Gamma$ of operations in the \hr-algebra and an  \mso transduction $h$ which makes the following diagram commute 
    \[
    \begin{tikzcd}
    \text{trees}
    \ar[dr,"f"']
    \ar[r,"h"]
    & \text{terms over $\Gamma$} 
    \ar[d,"{\text{value of a term}}"] \\ 
    & 
    \text{incidence representations of graphs}
    \end{tikzcd}
    \]
    
\end{proof}

\begin{fact}
    If a funcion  $f : \Cc \to \set{\text{yes, no}}$ is \mso definable, then it is recognizable. 
\end{fact}


==> simon.tex <==

    \subsubsection{Putting it all together}

    We now use the closure properties proved above to complete the proof of Theorem~\ref{thm:bounded-branchwidth-for-matroids}. 
    Consider an \mso transduction 
    \begin{align*}
    f : \Sigma^* \to \text{matroids}.
    \end{align*}
    Our goal is to prove that the image of $f$ has original tree decompositions.  Without loss of generality, we can assume that $f$ is an \mso interpretation, i.e.~it does not use copying or colouring. This is because the copying and colouring can be integrated into the input string.  
    
    
Define a \emph{derivative} of $f$ to be any string-to-multi-matroid function of the form
\begin{align*}
v \in \Sigma^* \quad \mapsto \quad f(uvw)/X\setminus Y
\end{align*}
for some fixed strings $u,w$ and some partition $X \cup Y$ of the positions in these strings. One of the derivatives is $f$ itself, this happens when the strings $u$ and $w$ are empty.

    \begin{lemma}\label{lem:residual-functions}
        There are finitely many derivatives of $f$.  
    \end{lemma}
    \begin{proof}
        Compositionality of \mso.
    \end{proof}


\begin{definition}
    \label{def:good-language}
    We say that a language $L \subseteq \Sigma^*$ is \emph{good} if for every derivative $g$ of $f$, the function class $\setbuild{g(v)}{$v \in L$}$ 
    has original tree decompositions.
\end{definition}

To prove Theorem~\ref{thm:bounded-branchwidth-for-matroids}, we will show that the class of good languages has the following three closure properties.
    \begin{enumerate}
        \item Every finite language is good.
        \item  The concatenation of two good languages is also good, i.e.~if $L$ and $K$ are good, then so is $L \cdot K$.
        \item There is a monoid homomorphism 
        \begin{align*}
        h : \Sigma^* \to M
        \end{align*}
        into a finite monoid such that the following condition is sufficient for $L^*$ being good:  $L$ is a good, and all words in $L$ are mapped by $h$ to the same element of $M$ which is furthermore an idempotent.
    \end{enumerate}

     The Factorization Forest Theorem of Imre Simon~\cite[Theorem 6.1]{simonFactorizationForestsFinite1990} says that any class of languages contained in $\Sigma^*$ that has the three closure  properties described above will necessarily contain the full language  $\Sigma^*$. Therefore, if we establish the three closure properties, we will know that $\Sigma^*$ is good, and therefore the image of $f$ has original tree decompositions, as in the conclusion of Theorem~\ref{thm:bounded-branchwidth-for-matroids}.

     Consider the first closure property, about every finite language being good. This is an immediate corollary of the fact that every finite class has original tree decompositions.

     \subparagraph*{Binary concatenation.}
     Consider now the second property, about good languages being closed under concatenation. Suppose then that $L_1$ and $L_2$ are good langaugages. We need to show that derivative $g$ of $f$, the 
     \begin{align*}
     \setbuild{ g(v_1v_2) } { $v_1 \in L_1$ and $v_2 \in L_2$}
     \end{align*}
     For each matroid in this class, consider the ordered parition into two parts $X_1$ and $X_2$, corresponding to the elements that have origins in $v_1$ and $v_2$ respectively. The residual list of this ordered partition consists of two multi-matroids, each one taken from the two classes 
     \begin{align*}
     \bigcup_{v_2 \in L_2}\setbuild{g(v_1v_2)@v_1 }{$ v_1 \in L_1$} \qquad      \bigcup_{v_1 \in L_1}\setbuild{g(v_1v_2)@v_2 }{$ v_2 \in L_2$}.
     \end{align*}
     By symmetry, we only show that the first class has original tree decompositions; the same argument will work for the second class. 
     Because each deriviative is \mso definable, it the above unions are in fact finite, and therefore it is enough to show that for every $v_2 \in L_2$ the class 
     \begin{align*}
        \setbuild{g(v_1v_2)@v_1 }{$ v_1 \in L_1$}
     \end{align*}
     has original tree decompositions.  By Lemma~\ref{lem:reduce-to-residuals} below, the above class has  original tree decompositions if and only if the same is true for
     \begin{align*}
     \setbuild{g(v_1v_2)}{$v_1 \in L_1$},
     \end{align*}
     and the latter class has original tree decompositions thanks to the  induction assumption, swince $v_1 \mapsto g(v_1v_2)$ is a derivative of $f$. It remains to state and prove the lemma. 

     \begin{lemma}\label{lem:reduce-to-residuals}
        Let $g$ be a derivative of $f$, let $u,w \in \Sigma^*$ and let $L \subseteq \Sigma^*$. Then the class of matroids 
        \begin{align*}
        \setbuild{g(uvw)}{$v \in L$}
        \end{align*}
        has original tree decompositions if and only if the class of multi-matroids 
        \begin{align*}
            \setbuild{g(uvw)@v}{$v \in L$}
        \end{align*}
        has original tree decompositions.
     \end{lemma}

     
     \subparagraph*{The idempotent step.} 
     We are left with the last closure property of good languages, namely that there 
     is a monoid homomorphism 
     \begin{align*}
     \varphi : \Sigma^* \to M
     \end{align*}
     into a finite monoid such that the following condition is sufficient for $L^*$ being good:  $L$ is a good, and all words in $L$ are mapped by $h$ to the same element of $M$ which is furthermore an idempotent. 
     The homomorphism $\varphi$ is chosen so that ... Suppose now that $L$ is good, and all words in $L$ have the same value under the homomorphism $\varphi$, which is furthermore idempotent. We need to show that for every derivative $g$ of $f$, the class
     \begin{align*}
        \setbuild{g(v_1 \cdots v_n)}{$v_1,\ldots,v_n \in L$} 
        \end{align*}
        has original tree decompositions. This is prove in multiple steps below, using the closure properties that we have collected so far. 
    \begin{enumerate}
        \item By the same argument as in the binary step, to prove that 
        \begin{align*}
        \setbuild{g(v_1 \cdots v_n)}{$v_1,\ldots,v_n \in L$} 
        \end{align*}
        has original tree decomposition, it is enough to show that for every fixed choices of $u,w \in L$, the class 
        \begin{align*}
            \setbuild{g(uv_1 \cdots v_nw)@\text{(origin in $v_1 \cdots v_n$)}}{$v_1,\ldots,v_n \in L$} 
            \end{align*}
        has original tree decompositions.  By assumption that all words in $L$ have the same value under the homomorphism $\varphi$, and the choice of this homomorphism, this class does not depend on the choice of $u,v$. In particular, we can use $u=v$ Furthermore, since the value assigned by the homomorphism to $u$ is idempotent, this class is equal to 
        \begin{align*}
            \setbuild{g(uuv_1 \cdots v_nu)@\text{(origin in $v_1 \cdots v_n$)}}{$v_1,\ldots,v_n \in L$}.
            \end{align*}
    \item   Let $u \in L$. By Lemma~\ref{lem:reduce-to-residuals}, the class from the previous item has original tree decompositions if and only if the same is true for 
    \begin{align*}
        \setbuild{g(uuv_1 \cdots v_nu)}{$v_1,\ldots,v_n \in L$}.
        \end{align*}
        \item Let $u$ be as in the previous item. Define a new function 
        \begin{align*}
        h(v) = g(uuvu) / \text{(origin in first copy of $u$)} \setminus \text{(origin in second and third copies of $u$)}.
        \end{align*}
        This function is a derivative of the original function $f$.
        Since the word $u$ is fixed, for every matroid in the class from the previous item, a constant sequence of contractions and deletions leads to a matroid in the class 
        \begin{align*}
        \setbuild{ h(v_1 \cdots v_n)}{$v_1,\ldots,v_n \in L$}.
        \end{align*}
        Therefore, by Corollary~\ref{cor:minor-dtd}, it is enough to find original tree decompositions for the class from this item.
        \item By Lemma~\ref{lem:connected-components}, it is enough to find original tree decompositions for the connected components of the class from the previous item, i.e.~for the class
        \begin{align*}
            \setbuild{ A }{\text{$A$ is a connected component of $h(v_1 \cdots v_n)$ for some $v_1,\ldots,v_n \in L$}}.
            \end{align*}
        
            \item In a matroid $A$ from the class in the previous item, consider the ordered partition $\le$ into elements that have origins in $v_1,\ldots,v_n$, respectively. This ordered partition is homogenous thanks to ..., and therefore it can be produced by \mso transduction thanks to Lemma~\ref{lem:define-homogeneous-order}. Therefore, to prove that the class from the previous item has original tree decompositions, it is enough to prove the same for
                \begin{align*}
                    \setbuild{ (A,\le)}{\text{$A$ is a connected component of $h(v_1 \cdots v_n)$ for some $v_1,\ldots,v_n \in L$}\\ \text{and $\le$ is the ordered partition into parts with origins in $v_1,\ldots,v_n$}}.
            \end{align*}
            \item By Lemma~\ref{lem:reconstruct-multi-matroid-from-list}, to prove that the class from the previous item has original tree decompositions, it is enough to prove the same for
            \begin{align*}
                \setbuild{ h(v_1 \cdots v_n) @ X}{\text{$v_1,\ldots,v_n \in L$ and there is some $i \in \set{1,\ldots,n}$ such that $X$ is the set of all} \\
                \text{elements with origin in $v_i$ in some connected component of $h(v_1 \cdots v_n)$}}.
        \end{align*}
            \item In a multi-matroid $h(v_1 \cdots v_n) @ X$ as in the previous item, all connected components are connected components of the multi-matroid $h(v_1 \cdots v_n) @ v_i$. Therefore, to prove that the class from the previous item has original tree decompositions, it is enough to prove the same for
            \begin{align*}
                \setbuild{ h(v_1 \cdots v_n) @ v_i}{\text{$v_1,\ldots,v_n \in L$ and  $ i \in \set{1,\ldots,n}$}}.
        \end{align*}
        \item The class in the previous item is equal to  
        \begin{align*}
        \bigcup_{\substack{n \in \set{1,\ldots}\\ i \in \set{1,\ldots,n}}} 
        \bigcup_{\substack{v_1,\ldots,v_{i-1} \in L\\
        v_{i+1},\ldots,v_{n} \in L}}   \setbuild{ h(v_1 \cdots v_n) @ v_i}{$v_i \in L$}.
        \end{align*}
        Because the function $h$ is \mso definable, the above union is in fact finite, i.e.~it is a finite union of sets of the form 
        \begin{align*}
            \setbuild{ h(uvw) @ v}{$v \in L$} 
        \end{align*}
        where the parameters $u$ and $w$ are finite concatenations of words in $L$. Therefore, it is enough to show that each such set has original tree decompositions. By Lemma~\ref{lem:reduce-to-residuals}, this is equivalent to showing that for every $u,w$ the set 
        \begin{align*}
            \setbuild{ h(uvw) }{$v \in L$} 
        \end{align*}
        has original tree decompositions, which is true by induction assumption, since $v \mapsto h(uvw)$ is a derivative of $f$. 
    \end{enumerate}
This completes the proof of the idempotent step, and therefore the proof that all languages are good, and therefore also the proof of Theorem~\ref{thm:definable-tree-decompositions-for-matroids}. 
We will show that the following class has original tree decompositions
\begin{align*}
    \setbuild{\residf u {vv_1 \cdots v_nv} w}{$v_1,\ldots,v_n$ have $h$-trees of\\ height at most $\ell$ and value $e$}.
    \end{align*}
    

    Consider the \mso transduction 
    \begin{align*}
    f : \Sigma^* \to \text{matroids}.
    \end{align*}
We assume without loss of generality that $f$ is an \mso interpretation, i.e.~it does not use copying or colouring. This is because for every \mso transduction whose domain is strings, there is another \mso transduction from strings that has the same image, and does not use copying or colouring. In a matroid, there is only one relation, namely the independence relation. This means that there are two \mso formulas that define $f$: one for the universe relation (one elements) and one for the independence relation (on sets). These formulas can be seen as two languages over the alphabet $\Sigma \times \set{0,1}$:
\begin{align*}
\setbuild{w \otimes \set{x}}{$x$ satisfies the universe formula}\\
\setbuild{w \otimes X}{$X$ is an independent set},
\end{align*} 
where $w \otimes X$ denotes the word obtained from $w$ by adding to each letter a bit that indicates if the position is in the set $X$. Take some monoid homomorphism 
\begin{align*}
h : (\Sigma \times 2)^* \to M
\end{align*}

\begin{lemma} \label{lem:idempotents-use} For every deterministic \mso transduction 
    \begin{align*}
    f : \Sigma^* \to \text{matroids}
    \end{align*}
    there is a monoid homomorphism 
    \begin{align*}
    h : \Sigma^* \to \myunderbrace{M}{a finite monoid}
    \end{align*}
    with the following property. Let
    \begin{align*}
    u,v_0,\ldots,v_{n},w \in \Sigma^*
    \end{align*}
    be words such that all $v_0,\ldots,v_n$ have the same image under $h$, and this image is an idempotent in the monoid $M$. Consider the multi-matroid
    \begin{align*}
    A = f(\underline{u} v_0 \cdots v_{n} \underline{w}),
    \end{align*}
    and define $Y_i$ to be the elements with origin in $v_i$ (these elements are also called elements of index $i$). Then 
    \begin{enumerate}
        \item \label{it:circuits-of-four-indexes} Suppose that  $x,y$ are elements of $A/Y_0$ with equal or consecutive indexes which can be connected by a circuit  that avoids indexes $1$ and $n$. Then $x$ and $y$ can be  connected by a circuit that uses at most four indexes.  

        \item \label{it:circuit-indexes-are-intervals} For every cycle in $A/Y_0$, the indexes used by this cycle form an interval in $\set{1,\ldots,n}$.
    \end{enumerate}
\end{lemma}
\begin{proof}
    The proof is based on two ingredients: (a) \mso can formalize matroid concepts such as contraction; and (b)  on words \mso corresponds to finite monoids. 
    We prove the two items separately, which will give two monoid homomorphisms. By pairing the two homomorphisms, we get a single homomorphism as in the statement of the lemma. 
    
\paragraph*{Short circuits.}  We  begin with item~\ref{it:circuits-of-four-indexes}. Let $u,v_0,\ldots,v_n,w$ and  $A$ be as in the lemma.  For $i \in \set{0,\ldots,n}$ let us write  $Y_i$ to be the elements of $A$ that have  index~$i$. Suppose that  $x,y$ are elements of $A/Y_0$ with equal or consecutive indexes that can be connected by a circuit in $A/Y_0$ that avoids indexes $1$ and $n$. We will show that $x$ and $y$ can be  connected by a circuit in $A/Y_0$ that uses at most four indexes.  

By symmetry, we assume that the index of $x$ is smaller or equal to the index of $y$. We will show that if $x$ and $y$ can be connected in $A/Y_0$ by a circuit  that avoids indexes $1$ and $n$, then they can be connected by a circuit in $A/Y_0$ where all indexes used are contained in the interval 
\begin{align}\label{eq:small-set-of-indices}
\set{\text{index of $x-1$},\ldots,\text{index of $y+1$}}.
\end{align}
If the indexes $i$ and $j$ differ by at most one, then this interval has size at most four.
The main idea is to use \mso to formalize the notions of connectivity and contraction. 
Consider the statement 
    \begin{itemize}
    \item[(*)] if we take the matroid $f(u v_0 \cdots v_n w)$ and contract all elements  in $Y_0$, then there exists a circuit that connects $x$ and $y$, and which avoids elements with origin in $Y_1$ and $Y_n$.
    \end{itemize}
    One can express (*) using  an \mso formula, which inputs a word $u v_0 \cdots v_n w$ with three distinguished sets $Y_0, Y_1, Y_n$ and two distinguished elements $x,y$. This formula depends only on the \mso transduction  $f$ that defines the matroid $A$ in terms of the input string.  The circuit that connects $x$ and $y$ while using only indexes in the set~\eqref{eq:small-set-of-indices} will be obtained by applying the following claim to the formula that defines (*).
    
    \begin{claim}\label{claim:mso-mso-swap-one} 
        Let $\varphi$ be an \mso formula, over the vocabulary of words over an alphabet $\Sigma$. There is a monoid homomorphism 
        \begin{align*}
        h : \Sigma^* \to M
        \end{align*}
        such that for every 
        \begin{align*}
            u,\myunderbrace{v_0,\ldots,v_{n}}{these elements have the same value under $h$, which is an idempotent}, w \in \Sigma^*.
        \end{align*}
    and every  positions $x \le y$, the following conditions are equivalent 
\[
\begin{tikzcd}
    u v_0 \cdots v_n w \models \varphi(Y_0, Y_1, x, y,  Y_n)     
\ar[d,Leftrightarrow]\\
u v_0 \cdots v_n w \models \varphi(Y_0, Y'_1, x, y,  Y'_n) 
\end{tikzcd}
\]
     where the sets $Y'_1$ is obtained from $Y'_1$ by adding all elements with index smaller than $x$ by at least two, and  $Y'_n$ is obtained from $Y_n$ by adding all elements with index  bigger than $y$ by at least two, as explained in the following picture: 
     \mypic{16}
    \end{claim}
\begin{proof}
    Compositionality of monadic second-order logic. Let $r \in \set{0,1,\ldots}$ be the quantifier rank of the formula $\varphi$, i.e.~the nesting depth of quantifiers. Let $h$ be the function that maps a word to the set of \mso sentences that are true in this word and have quantifier rank at most $r$. The classical result about \mso on words is that: (a) this function has finitely many possible values; and (b) there is a monoid structure on the image which turns $h$ into a monoid homomorphism. Therefore, $h$ can be seen as monoid homomorphism into a finite monoid. 
    
    Each of the two situations described in the statement of the lemma can be partitioned into several parts, such that the corresponding parts have the same values under $f$:
    \mypic{17}
    The parts (a), (e) and (h) are the same both in the top picture and the bottom picture. The remaining parts are equivalent by the assumption on independence. In fact, all of the remaining parts are equivalent, e.g. (c) at the top is equivalent to (f) at the top, but we only need the weaker property that (c) at the top is equivalent to (c) at the bottom, and likewise for the other parts.
\end{proof}
    \paragraph*{Indexes are intervals.} We now move to item~\ref{it:circuit-indexes-are-intervals} in the lemma, which says that for every circuit in $A/Y_0$, the indexes used are an interval in $\set{1,\ldots,n}$. Similarly to the previous item, we will use compositionality, as stated in the following claim. 
\begin{claim}\label{claim:mso-first-second} 
    Let $\varphi(X,Y)$ be an \mso formula, over the vocabulary of words over an alphabet $\Sigma$. There is a monoid homomorphism 
    \begin{align*}
    h : \Sigma^* \to M
    \end{align*}
    such that for every 
    \begin{align*}
        u,\myunderbrace{v_0,\ldots,v_{n}}{these elements have the same value under $h$, which is an idempotent}, w \in \Sigma^*.
    \end{align*}
and every   $X$ set of positions in $u v_0 \cdots v_i w$ disjoint with $Y_0 \cup \cdots \cup Y_i$, we have  
\[
\begin{tikzcd}
    u v_0 \cdots v_n w \models \varphi(X, Y_0)
    \ar[d,Leftrightarrow]\\
    u v_0 \cdots v_n w \models \varphi(X,Y_0 \cup \cdots \cup Y_{i-1}).
\end{tikzcd}
\]
\end{claim}
\begin{proof}
    Same proof as in Claim~\ref{claim:mso-mso-swap-one}, with the corresponding picture being 
    \mypic{18}
\end{proof}

Using the above claim, we  prove item~\ref{it:circuit-indexes-are-intervals} in the lemma: for  every circuit in $A/Y_0$, the indexes used are an interval in $\set{1,\ldots,n}$.  In other words, we need to show that if a circuit $X$ in $A/Y_0$ avoids some index $i \in \set{1,\ldots,n}$ and contains at least one element with index $>i$, then it cannot contain any elements of index $<i$. 
    
    Choose some basis $Z_0$ of the matroid $A|Y_0$, i.e.~some maximal independent set of elements of index zero. By definition of contraction, the elements of $A/Y_0$ are elements of nonzero index, and a set of such elements satisfies
    \begin{align*}
    X \text{ independent in } A/Y_0 
    \quad\text{iff}\quad
    X \cup Z_0 \text{ independent in } A.
    \end{align*}
    % Furthermore, the above condition does not dependent on the choice of basis $Z_0$, but this will not be important in the proof below. 
    Suppose that $X$ is a circuit in $A/Y_0$, which avoids some index $i$ and has at least one element $>i$. Since $X$ has at least one element of index $>i$, it follows that 
    \begin{align*}
        X \cap (Y_1 \cup \cdots \cup Y_{i-1})
    \end{align*}
    is a proper subset of $X$, and therefore it must be independent in $A/Y_0$, which means 
    \begin{align}\label{eq:z0cupcap}
        \myunderbrace{Z_0 \cup (X \cap (Y_1 \cup \cdots \cup Y_{i-1}))}{same thing as $(X \cup Z_0) \cap (Y_0 \cup \cdots \cup Y_{i-1})$} \text{ is independent in $A$}.
    \end{align}
    Consider the set $Z_0 \cup X$ in the matroid $A$. This set is dependent, since $X$ is a circuit in $A/Y_0$, however in~\eqref{eq:z0cupcap} we have proved that this set becomes independent after restricting it to the set $Y_0 \cup \cdots \cup Y_{i-1}$. Therefore, this set is dependent after contracting $Y_0 \cup \cdots \cup Y_{i-1}$, in the sense that:
    \begin{align}\label{eq:fist-dependence}
    X \setminus (Y_0 \cup \cdots \cup Y_{i-1}) \text{ is dependent in }A/(Y_0 \cup \cdots \cup Y_{i-1}).
    \end{align}
    The property above can be defined by a formula of \mso, which takes two arguments, as described below:
    \begin{align*}
        \myunderbrace{X \setminus (Y_0 \cup \cdots \cup Y_{i-1})}{first argument} \text{ is dependent in }A/(\myunderbrace{Y_0 \cup \cdots \cup Y_{i-1}}{second argument}).
    \end{align*} 
    We can therefore use  Claim~\ref{claim:mso-first-second}  to conclude  
    \begin{align*}
        X \setminus (Y_0 \cup \cdots \cup Y_{i-1}) \text{ is dependent in }A/Y_0.
        \end{align*}
    Since the $X$ was assumed to be a circuit in $A/Y_0$, this means that the above set cannot be a proper subset of $X$, which means that $X$ does not contain any elements of index $<i$.
    \end{proof}


    \begin{corollary}
        Let $h$ be the homomorphism from the previous lemma. Let $\Cc$ be a class of multi-matroids with original tree decompositions, let  $e$ be an idempotent in the target monoid of $h$, and let
        \begin{align*}
        u,v_0, w \in \Sigma^* \qquad h(v_0) = e.
        \end{align*}
        Then the class $\Dd$ of multi-matroids below as follows has original tree decompostions. A multi-matroid belongs to $\Dd$ if it  can be obtained by choosing some words $v_1,\ldots,v_n \in L$ that have image $e$ under $h$, taking the multi-matroid 
        \begin{align*}
            \residf u {v_0 v_0 v_1 \cdots v_n v_0} w,
        \end{align*}
        contractin the elements with origin in the first copy of $v_0$, and deleting the elements with origin in the remaining two copies of $v_0$.
    \end{corollary}





We now recall the  Factorization Forest Theorem of Imre Simon, which will be applied to  the monoid homomorphisms discussed in the above lemma and in Lemma~\ref{lem:idempotents-use}.
    Define a \emph{factorization tree} for a monoid to be  to be an ordered tree where leaves are labelled by monoid elements such that: (a) for  every non-leaf node, its label is the product, in the monoid, of the labels of its children;  and (b) if a node has at least three children, then all of these children have the same label, and this label is a monoid idempotent. Here is a picture of a factorization tree for the two element group:
    \mypic{19}
    The \emph{yield} of a factorization tree is the sequence of leaves, read from left to right. Define the \emph{height} of a tree to be the maximal number of edges on a root-to-leaf path, e.g.~the tree in the picture above has height 5.  We will use the following theorem 
    
    \begin{theorem}[Factorization Forest Theorem]
        For every finite monoid there exists some $k \in \set{1,2,\ldots}$ such that every sequence of monoid elements is the yield of some factorization tree of height at most $k$.    
    \end{theorem}
    

    \newcommand{\residuals}[1]{\underline{#1}}


    Apply Lemma~\ref{lem:idempotents-use} to $f$, yielding some monoid homomorphism
    \begin{align*}
    h : \Sigma^* \to M.
    \end{align*}
    Without loss of generality, we can assume that the monoid homomorphism refines the monoid homomorphism from Lemma~\ref{lem:residual-functions}, which means that the residual $\residf u v w$ depends only on $v$ and the monoid elements $h(u)$ and $h(w)$. We say that a word in $w \in \Sigma^*$ has a factorization tree of height at most $k$ if there is a factorization tree for the monoid $M$, whose yield is the sequence of monoid elements obtained by applying $h$ to the individual letters in $w$. 
    By induction on $k \in \set{0,1,\ldots}$, we will prove the following invariant: for every $u,w \in \Sigma^*$, the following set has original tree decompositions: 
    \begin{align*}
        \setbuild{\residf u v w}{$v$ has a factorization tree height at most $k$}.
    \end{align*}
    If we apply the invariant to $u=w$ being the empty word and $k$ being the minimal height of factorization forests needed to cover all words, we will get the desired result that the image of $f$ has original tree decompositions. By definition of factorization trees, it is enough to show that if 
    \begin{align*}
    \residuals L  \quad \eqdef \quad \setbuild{\residf u v w} {$v \in L$ and  $u,w \in \Sigma^*$}
    \end{align*}
    has original tree decompositions,    then the same is true for $\residuals{LL}$ and 
    \begin{align*}
     \residuals{\setbuild{v_1 v_2 \cdots v_n} {$v_1,\ldots,v_n \in L$  have the same idempotent image under $h$}}.
    \end{align*}

    

    \subsubsection{Binary step}
    In this section, we that if $L \subseteq \Sigma^*$ is such that $\residuals L$  has original tree decompositions, then the same is true for $\underline{LL}$. We will use the following straightforward observation.
     \begin{lemma}\label{lem:definable-tree-decompositions-on-dense-subset}
            Let $g : \Cc \to \Dd$ is an \mso encoding, and let $\Ee \subseteq \Dd$ be a class such that every input to $g$ has at least one output in $\Ee$. If $\Ee$ has original tree decompositions, then so does $\Cc$. 
        \end{lemma}
    \begin{proof}
        The natural idea would be to simply restrict $g$ to outputs from $\Ee$, but this is not necessarily possible, since we do not assume that $\Ee$ is definable in \mso. We work around this as follows. Take encoding 
        \begin{align*}
        f : \Ee \to \text{trees}
        \end{align*}
        and extend its domain to $\Ee$. The result is some 

    \end{proof}

    Let $\ell$ be an upper bound on the degree of all multi-matroids in $\residuals L$. Such an upper bound exists by Lemma~\ref{lem:residual-functions}. We will apply Lemma~\ref{lem:definable-tree-decompositions-on-dense-subset} to the (nondeterministic) operation 
    \begin{equation}
        \label{eq:residual-pairs}
        \begin{tikzcd}
            \myunderbrace{\residuals L}{$\Cc$}
            \ar[r,"g"]
            &
            \myunderbrace{
                \left(\txt{multi-matroids of \\ degree at most $\ell$}\right)^*
            }{$\Dd$}
            \end{tikzcd}
    \end{equation}
    defined as follows: for every input   multi-matroid $A$, then the possible outputs are all lists   $[A_1,A_2]$ of length two  that can be obtained by taking the residuals of some  partition of $A$ that has two equivalence classes of degree at most $\ell$. The subset $\Ee$ is $(\residuals L)^*$.  It remains to justify that the assumptions of Lemma~\ref{lem:definable-tree-decompositions-on-dense-subset} are met:
    \begin{enumerate}
        \item The operation $g$ is an \mso transduction. This is because an ordered partition with two equivalence classes can be represented by a nondeterministically chosen colouring of the input multi-matroid.
        \item The operation $g$ has a decoding. This is thanks to Lemma~\ref{lem:reconstruct-multi-matroid-from-list}.
        \item For every input, there is some output in $\Ee$. This is because 
        \begin{align*}
            \residf {u} {v_1} {v_2w} 
            \text{ and } 
            \residf {uv_1} {v_2} {w} 
            \quad \text{ are residuals of }\quad 
             \residf {u} {v_1 v_2} w,
            \end{align*}
        \item The subset $\Ee$ has original tree decompositions. This is by the assumption that $\residuals L$ has original tree decompositions, and because having original tree decompositions is preserved under taking lists.
    \end{enumerate}
    

    \subsubsection{Ideompotent step}
    In this section, we that if $e$ is an idempotent in the monoid used by $h$, and 
     $L \subseteq \Sigma^*$ is such that $\residuals L$  has original tree decompositions and all words in $L$ have value $e$, and all words in $L$ have the same idempotent  then the same is true for 
    \begin{align*}
        \residuals{\setbuild{v_1 v_2 \cdots v_n} {$v_1,\ldots,v_n \in L$  have the same idempotent image under $h$}}.
       \end{align*}
    By unfolding the definitions, this means that we need to show that there are original tree decompositions for the class
    \begin{align*}
        \bigcup_{u,v} \bigcup_{e}{\setbuild{\residf u {v_1 v_2 \cdots v_n} w } {$v_1,\ldots,v_n \in L$ and $h(v_1) = \cdots = h(v_n) = e$}},
    \end{align*}
    where $u,v$ in the union range over words in $\Sigma^*$ and $e$ ranges over idempotents in the finite monoid used by the homomorphism $h$. There are finitely many choices for $e$ by finiteness of the monoid, and there are finitely many non-equivalent choices for $u$ and $v$ by Lemma~\ref{lem:residual-functions}. Therefore, since having original tree decompositions is preserved under taking unions, it is enough to show that for every choice of $u,v$ and $e$, the class 
    \begin{align}
    \label{eq:idempotent-class-to-show}
    \setbuild{\residf u {v_1 v_2 \cdots v_n} w } {$v_1,\ldots,v_n \in L$ and $h(v_1) = \cdots = h(v_n) = e$}
    \end{align}
    has original tree decompositions. 
    
    
\begin{lemma}
    Without loss of generality, in~\eqref{eq:idempotent-class-to-show} we can assume 
    \begin{align*}
    h(u)e = h(u) \quad \text{and} \quad eh(w)=h(w).
    \end{align*}
\end{lemma}
\begin{proof}
    We need to show that if there are original tree decompositions for every class as in~\eqref{eq:idempotent-class-to-show} where the parameters $u,w$ and $e$ satisfy the equations from the lemma, then there are also original tree decompositions for every class where the parameters  do  not necessarily satisfy the equations. 
    
    Let $\Cc$ be any class as in~\eqref{eq:idempotent-class-to-show}, for parameters which do not necessarily satisfy the equations from this lemma. 
    Let  $\Ee$  be the union of $\residuals L$ and all the  languages as in~\eqref{eq:idempotent-class-to-show}, subject to parameters  that do satisfy the  equations in the lemma. Assuming that $\Ee$, and therefore also $\Ee^*$, has original tree decompositions, we will show that  $\Cc$ has original tree decompositions. 
    By the same argument as in the idempotent step,  there is an \mso encoding from $\Cc$ to lists of multi-matroids of degree at most $\ell$, such that for every input 
    \begin{align*}
    \residf u {v_1 \cdots v_n} w \in \Cc,
    \end{align*}
     there is at least one in $\Ee^*$, namely 
     \begin{align*}
        [
            \myunderbrace{\residf u {v_1 } {v_2 \cdots v_nw}}{in $\Ee$ because in  $\residuals L$}, 
        \myunderbrace{\residf  {uv_1 } {v_1 \cdots v_n}{w}}{in $\Ee$ because \\ 
        $h(v_1)=h(v_n)=e=ee$\\ implies \\
        $h(uv_1)e =  h(uv_1)$\\ and \\
$eh(v_nuv) =  h(v_nu)$ 
        },
        \myunderbrace{\residf {u v_1  \cdots v_{n-1}} {v_n} w}{in $\Ee$ because in  $\residuals L$}
        ]
        \end{align*}
        Therefore, we can apply Lemma~\ref{lem:definable-tree-decompositions-on-dense-subset} to conclude that $\Cc$ has original tree decompositions.
\end{proof}

Thanks to the above lemma, it remains to show that if $u,v$ and $e$ satisfy the two equations in the lemma, then 
\begin{align*}
    \Cc =     \setbuild{\residf u {v_1 v_2 \cdots v_n} w } {$v_1,\ldots,v_n \in L$ and $h(v_1) = \cdots = h(v_n) = e$}
    \end{align*}
    has original tree decompositions. 
Choose some $v_* \in \Sigma^*$ that has value $e$ under $h$. Consider the class
\begin{align}\label{eq:idempotent-induction-step-v*}
    \setbuild{\residf u {v_* v_1 \cdots v_n v_*} w}{$v_1,\ldots,v_n \in L$}.
    \end{align}
Every multi-matroid in~\eqref{eq:idempotent-induction-step} is a residual of some  multi-matroid in~\eqref{eq:idempotent-induction-step-v*}. Therefore, by Lemma~\ref{lem:residuals}, it enough to show that the class~\eqref{eq:idempotent-induction-step-v*} has original tree decompositions.
Define 
\begin{align*}
    \residf u {v_* v_1 \cdots v_n v_*} w _{/v_*}
\end{align*}
to be  the multi-matroid obtained from 
\begin{align*}
    \residf u {v_* v_1 \cdots v_n v_*} w
\end{align*}
by contracting all elements which have origin in either  of the two copies of $v_*$. Every multi-matroid in~\eqref{eq:idempotent-induction-step-v*} admits a sequence of contractions of bounded length that leads to a multi-matroid in
\begin{align}\label{eq:idempotent-induction-step-v*-contracted}
    \setbuild{\residf u {v_* v_1 \cdots v_n v_*} w_{/v_*}}{$v_1,\ldots,v_n \in L$}.
    \end{align}
Therefore, by Lemma~\ref{lem:decontract-elements}, to show that~\eqref{eq:idempotent-induction-step-v*} has original tree decompositions, it is enough to show that 


